Say Less, Mean Better: Training-Free Verbosity Control for Language Models

Large language models (LLMs) often generate responses longer than necessary, increasing inference latency and computational cost. While prompting can encourage conciseness, controlling output length without compromising response completeness remains challenging. Aggressive early stopping can reduce generation costs but risks terminating responses prematurely. We introduce MinimalLM, a training-free framework for reliable verbosity control that combines uncertainty-aware, length-dependent stop-token adjustment with structural completeness guardrails. MinimalLM separates the decision of when to stop from whether stopping is structurally appropriate, coordinating response-level instructions, decoding-time intervention, and completion checks without modifying model parameters or requiring auxiliary models. We evaluate MinimalLM across three open-source LLMs and 330 questions, producing 5,940 responses across baseline and ablation configurations. MinimalLM reduces generated tokens by 47.6%, accelerates individual responses by 19-68%, and eliminates structurally truncated outputs in the primary evaluation. Despite substantial token savings, it achieves an average quality score of 8.04/10, compared with 8.42/10 for unmodified models and 6.46/10 for length-matched truncation. Evaluations across diverse subject domains (such as healthcare, programming, law, and science) demonstrate robust efficiency gains, while ablations establish the complementary roles of decoding control and completeness constraints. Our findings highlight that efficient generation requires more than producing fewer tokens: it requires controlling when generation ends while preserving response integrity. MinimalLM offers a lightweight, training-free approach toward this goal.

==> languages_rows.tex <==
English & 40.2 & 79.0 & 47.5 & 0.0 & 12.0 \\
Arabic & 37.9 & 70.7 & 44.8 & 1.0 & 13.3 \\
Chinese & 36.5 & 75.3 & 46.3 & 0.7 & 8.0 \\
French & 40.0 & 77.3 & 45.3 & 0.7 & 11.7 \\
German & 40.1 & 76.3 & 46.5 & 0.3 & 10.3 \\
Spanish & 39.3 & 79.3 & 45.3 & 0.3 & 8.3 \\
Russian & 40.0 & 77.7 & 45.5 & 0.3 & 8.0 \\
\midrule
\textbf{s} & 39.0 & 76.1 & 45.6 & 0.6 & 9.9 \\

